DuaLight: Enhancing Traffic Signal Control by Leveraging Scenario-Specific and Scenario-Shared Knowledge

Reinforcement learning has been revolutionizing the traditional traffic signal control task, showing promising power to relieve congestion and improve efficiency. However, the existing methods lack effective learning mechanisms capable of absorbing dynamic information inherent to a specific scenario and universally applicable dynamic information across various scenarios. Moreover, within each specific scenario, they fail to fully capture the essential empirical experiences about how to coordinate between neighboring and target intersections, leading to sub-optimal system-wide outcomes. Viewing these issues, we propose DuaLight, which aims to leverage both the experiential information within a single scenario and the generalizable information across various scenarios for enhanced decision-making. Specifically, DuaLight introduces a scenario-specific experiential weight module with two learnable parts: Intersection-wise and Feature-wise, guiding how to adaptively utilize neighbors and input features for each scenario, thus providing a more fine-grained understanding of different intersections. Furthermore, we implement a scenario-shared Co-Train module to facilitate the learning of generalizable dynamics information across different scenarios. Empirical results on both real-world and synthetic scenarios show DuaLight achieves competitive performance across various metrics, offering a promising solution to alleviate traffic congestion, with 3-7\% improvements. The code is available under: https://github.com/lujiaming-12138/DuaLight.

==> 1-intro-dualight-plus.tex <==

% \jqruan{see comments}
% \jqruan{
% 读起来很别扭，用词比较复杂 陈述不够简洁，读起来很容易抓不到重点(也许是我对此不熟悉的缘故)
% 整体思路ok的：设置背景、介绍已有方法的不足、引出自己的亮点、summarize
% 能否精简第三段，是不是太冗长
% maybe 分item总结贡献会让读者更清晰get到你的novelty
% }
% 做了以下修改：

% 第一段：
% Traffic congestion is a pressing issue in metropolises, causing delays, increasing energy consumption, and reducing commuting comfort. This has led to urgent research on traffic signal control (TSC) to ease urban gridlock. （请把对应的参考文献加上，下面也是 不再赘述）

% 第二段：
% Conventional traffic-engineering-based methods, based on expert knowledge or intersection observations, struggle to adapt to the changing traffic patterns and coordinate strategies across multiple intersections. Recently, the emphasis of TSC has shifted towards deep reinforcement learning (DRL) methods, which can learn from intersection observations, eliminating the need for unrealistic assumptions about traffic-engineering-based models.

% 第三段：这段太长了(不过我刚check了几篇TSC的经典工作，大家写的都挺长的，but 我还是想下面精简一下，你批判性接收建议)
% DRL-based TSC can be divided into: 1) \textbf{Single-agent solution.} These methods can adaptively control based on observations such as queue lengths of each lane at intersections, through the design of certain network structures. However, they often require specialized expertise, and neglect coordination among multiple intersections. (此处不建议说：只关注到单个路口，因为单智能体接收的是全局的状态[global message]，输出的是联合动作；；如果非要说协作的话，感觉单智能体拿到所有路口的观测，似乎是跟所有路口都在协作)，我这里multiple intersections想表达的其实 是 忽略了特定范围内or子区内应有的协作，如果想不到 合适的说法，先不要改
% 其实单智能体一个致命的缺陷是：当随着状态动作空间的增大，解空间会呈现指数级的增长，导致要得到最优解会很棘手，应该就是第三段我留track中的comments的那句话表达出的缺点
% 2) \textbf{Multi-agent solution.} 
% A line of research treats each intersection as an independent agent and trains it in a centralized manner. However, they often fail to consider the coordination across neighboring intersections.
% Another line of research focuses on message aggregation by integrating observations of the target and the neighboring intersections, from both a spatial and spatiotemporal perspective, attaining coordinated control.
% Despite their potential, these methods often overfit to a single scenario, limiting their transferability to unseen scenarios, and struggling to extract generalized dynamical information from diverse scenarios.

% 第四段：
% Viewing these issues, we propose \textbf{DuaLight}, a novel framework comprised of two modules: Dual-experiential Weight and Co-Train, which enables concurrent learning from both the scenario-specific experiential information and the universal dynamics information across multiple scenarios.
% Specifically, the Dual-experiential Weight mechanism consists of two parts: Intersection-wise and Feature-wise modules. These modules can learn the environmental dynamic information about the neighbors and self-features within the scenario during training, while assigning distinct environment experience weights, providing a more fine-grained understanding of different intersections for the model.
% Additionally, the \textbf{Co-Train} module facilitates joint learning across multiple scenarios by allowing a subset of the model's parameters to be trained concurrently. This module helps the model extract the underlying dynamics information across diverse scenarios.

% 第五段
% The contributions of this paper are threefold.
% \begin{itemize}
    %\item As far as we know, we are the first to introduce the dual-experiential weight module to TSC, enabling the learning of the environmental dynamic information about neighbors and self-features within a particular scenario during training.
    % \item We propose the Co-Train module, allowing the model to be trained across multiple scenarios, and extracting the generalized dynamic information across different scenarios.
    % \item Empirical evaluations on both real-world and synthetic scenarios show DuaLight achieves competitive performance across various metrics.
% \end{itemize}


\vspace{-10pt}
\section{Introduction}
%background
Traffic congestion has emerged as a pressing issue in metropolises, leading to protracted travel and waiting time, heightened energy consumption, and diminished commuting comfort
\cite{levinson1998speed,tirachini2013estimation,economist2014cost,schrank20152015}.
Consequently, traffic signal control (TSC) has increasingly become a focal point of research, presenting an efficacious approach to alleviating such urban gridlock \cite{wei2019survey}.

Recently, the paradigm of TSC has predominantly shifted towards  deep reinforcement learning (RL) \cite{sutton2018reinforcement}. Such learning-based approaches \cite{li2016traffic,liang2018deep} can ``learn'' to give optimal actions directly based on the observation of intersections, which has proved its superiority over the conventional traffic-engineering-based methods such as SCATS and SCOOT \cite{roess2004traffic, hunt1982scoot,lowrie1990scats,gershenson2004self}, which are static models based on assumptions that could be unrealistic in front of the traffic dynamics.  
% traditional methods 需要假设，不是learningbase的
%Conventional traffic-engineering-based methods \cite{roess2004traffic, hunt1982scoot,lowrie1990scats,gershenson2004self} typically preconfigure control logic based on expert prior knowledge or select corresponding strategies based on observations of intersections. However, these methods are usually based on rigid assumptions such as uniform arrival rate that may not hold in real-life scenarios, thus lacking sufficient adaptability to cope with dynamic traffic situations.
% \hl{These methods tend to be shortsighted, struggling to account for the long-term impact on the system, and lacking the capacity for adaptive adjustment of coordinated strategies across multiple intersections.}
%Recently, the paradigm of TSC has predominantly shifted towards methods that utilize deep reinforcement learning (RL) %, with a specific emphasis on deep reinforcement learning
%\cite{sutton2018reinforcement}. These approaches \cite{li2016traffic,liang2018deep} learn to give optimal actions directly based on the observation of intersections, eliminating the need for unrealistic assumptions about control models. 
% Essentially, a TSC system based on RL first observes the traffic conditions, then generates and executes different actions (i.e., traffic control plans). Subsequently, it learns and adjusts strategies based on environmental feedback.
% RL-based solution: 分为两条技术路线，合作或多场景
Currently, there are two state-of-the-art solutions emerging in RL-based TSC: (1) cooperation among multi-agents and (2) learning via multi-scenarios.%, as concluded in Fig. \ref{fig:intro-two-sota}. 
%%\jiang{下面两个模块的顺序换成与title和方法里一致，先介绍weight再介绍co-train}

The first focuses on the cooperation of multiple intersections in one single \textit{scenario} (a simulation environment containing a set of intersections). With each intersection as an agent, multi-agent RL (MARL) \cite{mnih2016asynchronous,schulman2017proximal} have been developed. Most of the MARL-based TSC try to advocate cooperation by aggregating the information of the agents: they integrate the state of the target intersection with its neighboring intersections' states, either spatially \cite{van2016coordinated,wei2019colight} or spatiotemporally \cite{wang2020stmarl,wu2021dynstgat}, based on GNN \cite{wei2019colight} or GNN+LSTM/TCN to additionally capture long-range dependency \cite{wu2021dynstgat}, respectively. %, e.g., CoLight \cite{wei2019colight} used graph attention networks (GAT) \cite{velivckovic2017graph}. % with the objective of attaining coordinated control across multiple intersections.
Despite their potential, these approaches ignore that \textbf{how to coordinate with neighbors differs from scenarios}: training the model in only one particular scenario may lead to a local optimum due to overfitting, as discussed in \cite{jiang2023a}. 

%and do not possess an effective mechanism for extracting generalized dynamical information from diverse scenarios. 

The second type focuses on learning across multiple scenarios, such that the model could be more general for various regions or cities. 
To achieve this, different techniques such as meta RL \cite{zhang2020generalight,zang2020metalight}, attention mechanism \cite{oroojlooy2020attendlight} and standardization of intersections \cite{jiang2023a} have been proposed. For instance, MetaLight \cite{zang2020metalight} proposed a meta gradient learner through different datasets, and GESA \cite{jiang2023a} proposed a plug-and-play mapping module to enable multi-scenario co-training. These methods offer a potential solution to the overfitting problem mentioned before. 
However, they are all single-agent based, meaning one agent controls all the intersections, which may be an easy start for multi-scenario learning.
%从这里开始引出多场景协作的工作，然后陈述一下他的缺点：
MetaGAT \cite{lou2022meta} extended MetaLight to the multi-agent version by simply adding GAT in multi-scene training. 
However, these methods overlook that \textbf{how to utilize the unique knowledge of each scenario to facilitate the cooperation}: can we design an explicit mechanism for modeling experiential information within a single scenario?
%%\jiang{也可以抛出一个问题：比如如何利用场景内独特的 Knowledge来帮助协作}
%  some methods \cite{zhang2020generalight,zang2020metalight} use the Meta RL \cite{finn2017model} framework, with the aim of training models within existing scenarios and quickly transferring them to new scenarios. %Others tried multi-head attention mechanism \cite{oroojlooy2020attendlight} or standardization of intersections \cite{jiang2023a}.
%However, these methods have unstable performance and lack the ability to utilize dynamic information from experience within a single scenario.

% Solutions employing single-agent methods \cite{ault2019learning,ault2021reinforcement} can adaptively control based on observations such as queue lengths of each lane at intersections, through the design of certain network structures \cite{zheng2019learning,chen2020toward}. Nonetheless, the design of such model structures calls for specialized expertise, and their focus is narrowly concentrated on enhancing the traffic situation at individual intersections. And they are incapable of coordinating control among multiple intersections.
% Hence, multi-agent solutions \cite{mnih2016asynchronous,schulman2017proximal} have been developed. Some methods \cite{prashanth2010reinforcement,abdulhai2003reinforcement} 
% % \jqruan{pay attention to here, the detailed comments}
% directly train a centralized agent by using the observations of all intersections in a scenario as input to the model and providing a decision for each intersection. However, \hl{the complexity of these methods increases as the number of intersections increases, and they may fall into the sub-optimal solution due to the curse of dimension in joint action space.}
% In addition, some alternate methods consider each intersection as an individual agent. Through information aggregation, these methods integrate the state of the target intersection with the states of neighboring intersections, from both a spatial \cite{van2016coordinated,wei2019colight} or spatiotemporal \cite{wang2020stmarl,wu2021dynstgat} perspective, with the objective of attaining coordinated control across multiple intersections. Despite their potential, these approaches carry inherent drawbacks, e.g., training the model in only one particular scenario may lead to overfitting, making it difficult for the model to be effectively transferred to new scenarios. Furthermore, they do not possess an effective mechanism for extracting generalized dynamical information from diverse scenarios.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/intro.pdf}
    \caption{(1) Global knowledge from co-training, and (2) scenario-specific experiential knowledge formed as weights.}
    \label{fig:intro}
 % \vspace{-15pt}
\end{figure}
% \vspace{-10pt}


% \revise{To conclude, there is so far no work guiding how to coordinate multi-agent across multi-scenario. \hl{It is challenging since simply putting a multi-agent model in a multi-scenario learning setting could experience devastatingly unstable training, which has already taken shape in the single-agent version, i.e., MetaLight.} To encourage a long-term dynamic, introducing temporal modules such as LSTM is expected to aggravate the unstable learning, given the history is already unstable. To this end, this work is dedicated to solving the following research question: \textbf{how to coordinate multi-agent across multi-scenario stably and with the ability to reserve long-term experience}.}

%To address the drawbacks of these two types of models, 
To tackle these challenges, we propose \textbf{DuaLight} with two modules: \textbf{scenario-shared co-train} and \textbf{scenario-specific experiential weights}. %This innovative framework enables concurrent learning from both the universal dynamics information across multiple scenarios and the environmental experiential information within a single scenario. 
%We formulate the coordination parameters as the intersection-wise and feature-wise weights, guiding how to aggregate neighboring intersections' information and different observation features, respectively.
As shown in Fig \ref{fig:intro}: (1) \re{Some knowledge about the traffic underlining mechanisms is universal and commonly shared across various scenarios, for example, the flow is periodic, there are the potential morning/evening peak, and the merging and diversion of traffic flow along the network affect the traffic}. Co-Train module enables multi-scenario joint learning \re{of such global knowledge}. To encourage stability, only a \textbf{subset} of the model's parameters is trained concurrently, yet the essential coordination parameters are learned within each scenario. (2) \re{Some knowledge is scenario-specific: for example, each scenario has its unique distribution of the traffic flow, some tend to have more morning peaks and others more evening peaks, etc. This will affect different cooperation patterns from traffic lights.}  The experiential weight module defines the coordination parameters as the intersection-wise and feature-wise weights, guiding how to aggregate neighboring intersections' information and different observation features, respectively. The two weights are trained after observing a whole episode, capturing the long-term experiences. 

%This module can learn the environmental dynamic information about the neighbors and self-features within the scenario during training, which helps the model learn information that facilitates decision-making in a particular scenario. Specifically, this module can strengthen the experience information within a certain scenario by weighting the current neighbor observations and self-intersection observations.
%Additionally,  This module ensures the model's ability to extract the underlying dynamics information inherent across diverse scenarios.

The combination of these two modules encourages the model to learn and balance the shared dynamic information across multiple scenarios and the dynamic experiential information within a particular scenario, thus enabling the model to learn an effective representation to assist decision-making. This simple and effective dual design also supports our extension of using the neighbors \textbf{even from other scenarios}, which is a novel and promising discovery, as it can learn from similar intersections in other scenarios to further improve the ability of signal control.

%%\jiang{最后列一下贡献点} check
In summary, this paper has three main contributions:
\begin{itemize}
    \item To the best of our knowledge, we are the first that considers both scenario-common and scenario-specific information by co-train module and experiential weight module, respectively. This design also enables us to discover the potential of aggregating neighbors across scenarios. Overall, we coordinate multi-agents better across multi-scenario.
    \item Specifically, we design the scenario-specific experiential weights that encourage modeling the influence of neighbors and input features, adaptive to different scenarios. 
    \item We conduct experiments in both real-world and synthetic scenarios: DuaLight has the fastest and the most stable training and achieved the best results with 3-7\% improvements.
\end{itemize}
%First, the experiential weight module, which can learn the environmental dynamic information about neighbors and self-features within a particular scenario during training. Second, the Co-Train module, which enables the model to be trained across multiple scenarios, aims to learn the general dynamic information across different scenarios. Finally, we conduct experiments in both real-world and synthetic scenarios, where DuaLight achieved the best results or results close to the best across various metrics and scenarios.


==> 1-intro.tex <==

% \jqruan{see comments}
% \jqruan{
% 读起来很别扭，用词比较复杂 陈述不够简洁，读起来很容易抓不到重点(也许是我对此不熟悉的缘故)
% 整体思路ok的：设置背景、介绍已有方法的不足、引出自己的亮点、summarize
% 能否精简第三段，是不是太冗长
% maybe 分item总结贡献会让读者更清晰get到你的novelty
% }
% 做了以下修改：

% 第一段：
% Traffic congestion is a pressing issue in metropolises, causing delays, increasing energy consumption, and reducing commuting comfort. This has led to urgent research on traffic signal control (TSC) to ease urban gridlock. （请把对应的参考文献加上，下面也是 不再赘述）

% 第二段：
% Conventional traffic-engineering-based methods, based on expert knowledge or intersection observations, struggle to adapt to the changing traffic patterns and coordinate strategies across multiple intersections. Recently, the emphasis of TSC has shifted towards deep reinforcement learning (DRL) methods, which can learn from intersection observations, eliminating the need for unrealistic assumptions about traffic-engineering-based models.

% 第三段：这段太长了(不过我刚check了几篇TSC的经典工作，大家写的都挺长的，but 我还是想下面精简一下，你批判性接收建议)
% DRL-based TSC can be divided into: 1) \textbf{Single-agent solution.} These methods can adaptively control based on observations such as queue lengths of each lane at intersections, through the design of certain network structures. However, they often require specialized expertise, and neglect coordination among multiple intersections. (此处不建议说：只关注到单个路口，因为单智能体接收的是全局的状态[global message]，输出的是联合动作；；如果非要说协作的话，感觉单智能体拿到所有路口的观测，似乎是跟所有路口都在协作)，我这里multiple intersections想表达的其实 是 忽略了特定范围内or子区内应有的协作，如果想不到 合适的说法，先不要改
% 其实单智能体一个致命的缺陷是：当随着状态动作空间的增大，解空间会呈现指数级的增长，导致要得到最优解会很棘手，应该就是第三段我留track中的comments的那句话表达出的缺点
% 2) \textbf{Multi-agent solution.} 
% A line of research treats each intersection as an independent agent and trains it in a centralized manner. However, they often fail to consider the coordination across neighboring intersections.
% Another line of research focuses on message aggregation by integrating observations of the target and the neighboring intersections, from both a spatial and spatiotemporal perspective, attaining coordinated control.
% Despite their potential, these methods often overfit to a single scenario, limiting their transferability to unseen scenarios, and struggling to extract generalized dynamical information from diverse scenarios.

% 第四段：
% Viewing these issues, we propose \textbf{DuaLight}, a novel framework comprised of two modules: Dual-experiential Weight and Co-Train, which enables concurrent learning from both the scenario-specific experiential information and the universal dynamics information across multiple scenarios.
% Specifically, the Dual-experiential Weight mechanism consists of two parts: Intersection-wise and Feature-wise modules. These modules can learn the environmental dynamic information about the neighbors and self-features within the scenario during training, while assigning distinct environment experience weights, providing a more fine-grained understanding of different intersections for the model.
% Additionally, the \textbf{Co-Train} module facilitates joint learning across multiple scenarios by allowing a subset of the model's parameters to be trained concurrently. This module helps the model extract the underlying dynamics information across diverse scenarios.

% 第五段
% The contributions of this paper are threefold.
% \begin{itemize}
    %\item As far as we know, we are the first to introduce the dual-experiential weight module to TSC, enabling the learning of the environmental dynamic information about neighbors and self-features within a particular scenario during training.
    % \item We propose the Co-Train module, allowing the model to be trained across multiple scenarios, and extracting the generalized dynamic information across different scenarios.
    % \item Empirical evaluations on both real-world and synthetic scenarios show DuaLight achieves competitive performance across various metrics.
% \end{itemize}

\section{Introduction}
%background
Traffic congestion has emerged as a pressing issue in metropolises, leading to protracted travel and waiting time, heightened energy consumption, and diminished commuting comfort
\cite{levinson1998speed,tirachini2013estimation,economist2014cost,schrank20152015}.
Consequently, traffic signal control (TSC) has increasingly become a focal point of research, presenting an efficacious approach to alleviating such urban gridlock \cite{wei2019survey}.

Recently, the paradigm of TSC has predominantly shifted towards  deep reinforcement learning (RL) \cite{sutton2018reinforcement}. Such learning-based approaches \cite{li2016traffic,liang2018deep} can ``learn'' to give optimal actions directly based on the observation of intersections, which has proved its superiority over the conventional traffic-engineering-based methods such as SCATS and SCOOT \cite{roess2004traffic, hunt1982scoot,lowrie1990scats,gershenson2004self} since they are known as static models based on assumptions that could be unrealistic in front of the traffic dynamics.  
% traditional methods 需要假设，不是learningbase的
%Conventional traffic-engineering-based methods \cite{roess2004traffic, hunt1982scoot,lowrie1990scats,gershenson2004self} typically preconfigure control logic based on expert prior knowledge or select corresponding strategies based on observations of intersections. However, these methods are usually based on rigid assumptions such as uniform arrival rate that may not hold in real-life scenarios, thus lacking sufficient adaptability to cope with dynamic traffic situations.
% \hl{These methods tend to be shortsighted, struggling to account for the long-term impact on the system, and lacking the capacity for adaptive adjustment of coordinated strategies across multiple intersections.}
%Recently, the paradigm of TSC has predominantly shifted towards methods that utilize deep reinforcement learning (RL) %, with a specific emphasis on deep reinforcement learning
%\cite{sutton2018reinforcement}. These approaches \cite{li2016traffic,liang2018deep} learn to give optimal actions directly based on the observation of intersections, eliminating the need for unrealistic assumptions about control models. 
% Essentially, a TSC system based on RL first observes the traffic conditions, then generates and executes different actions (i.e., traffic control plans). Subsequently, it learns and adjusts strategies based on environmental feedback.

% RL-based solution: 分为两条技术路线，合作或多场景
Currently, there are two state-of-the-art solutions emerging in RL-based TSC: (1) cooperation among multi-agents and (2) learning via multi-scenarios, as concluded in Figure \ref{fig:intro-two-sota}. 
%%\jiang{下面两个模块的顺序换成与title和方法里一致，先介绍weight再介绍co-train}

The first focuses on the cooperation of multiple intersections in one single \textit{scenario} (a simulation environment containing a set of intersections). With each intersection as an agent, multi-agent RL (MARL) \cite{schulman2017proximal,su2023emvlight,ault2021reinforcement,yu2022surprising} have been developed. Most of the MARL-based TSC try to advocate cooperation by aggregating the information of the agents: they integrate the state of the target intersection with its neighboring intersections' states, either spatially \cite{van2016coordinated,wei2019colight} or spatiotemporally \cite{wang2020stmarl,wu2021dynstgat}, based on GNN \cite{wei2019colight} or GNN+LSTM/TCN to additionally capture long-range dependency \cite{wu2021dynstgat}, respectively.%, e.g., CoLight \cite{wei2019colight} used graph attention networks (GAT) \cite{velivckovic2017graph}. % with the objective of attaining coordinated control across multiple intersections.
Despite their potential, these approaches ignore that \textbf{how to coordinate with neighbors over time differs from scenarios}: training the model in only one particular scenario may lead to a local optimum due to overfitting, as discussed in \cite{jiang2023a}. 

%and do not possess an effective mechanism for extracting generalized dynamical information from diverse scenarios. 

The second type focuses on learning across multiple scenarios, such that the model could be more general for various regions or cities. 
To achieve this, different techniques such as meta RL \cite{zhang2020generalight,zang2020metalight}, attention mechanism \cite{oroojlooy2020attendlight} and standardization of intersections \cite{jiang2023a} have been proposed. For instance, MetaLight \cite{zang2020metalight} proposed a meta gradient learner through different datasets, and GESA \cite{jiang2023a} proposed a plug-and-play mapping module to enable multi-scenario co-training. These methods offer a potential solution to the overfitting problem mentioned before. 
However, they are all single-agent based, meaning one agent controls all the intersections, which may be an easy start for multi-scenario learning.
%从这里开始引出多场景协作的工作，然后陈述一下他的缺点：
MetaGAT \cite{lou2022meta} extended MetaLight to the multi-agent version by simply adding GAT in multi-scene training. 
However, these methods overlook that \textbf{how to utilize the unique knowledge of each scene to facilitate the cooperation}: \hl{can we design an explicit mechanism for modeling experiential information within a single scene?}
%%\jiang{也可以抛出一个问题：比如如何利用场景内独特的 Knowledge来帮助协作}
%  some methods \cite{zhang2020generalight,zang2020metalight} use the Meta RL \cite{finn2017model} framework, with the aim of training models within existing scenarios and quickly transferring them to new scenarios. %Others tried multi-head attention mechanism \cite{oroojlooy2020attendlight} or standardization of intersections \cite{jiang2023a}.
%However, these methods have unstable performance and lack the ability to utilize dynamic information from experience within a single scenario.

% Solutions employing single-agent methods \cite{ault2019learning,ault2021reinforcement} can adaptively control based on observations such as queue lengths of each lane at intersections, through the design of certain network structures \cite{zheng2019learning,chen2020toward}. Nonetheless, the design of such model structures calls for specialized expertise, and their focus is narrowly concentrated on enhancing the traffic situation at individual intersections. And they are incapable of coordinating control among multiple intersections.
% Hence, multi-agent solutions \cite{mnih2016asynchronous,schulman2017proximal} have been developed. Some methods \cite{prashanth2010reinforcement,abdulhai2003reinforcement} 
% % \jqruan{pay attention to here, the detailed comments}
% directly train a centralized agent by using the observations of all intersections in a scenario as input to the model and providing a decision for each intersection. However, \hl{the complexity of these methods increases as the number of intersections increases, and they may fall into the sub-optimal solution due to the curse of dimension in joint action space.}
% In addition, some alternate methods consider each intersection as an individual agent. Through information aggregation, these methods integrate the state of the target intersection with the states of neighboring intersections, from both a spatial \cite{van2016coordinated,wei2019colight} or spatiotemporal \cite{wang2020stmarl,wu2021dynstgat} perspective, with the objective of attaining coordinated control across multiple intersections. Despite their potential, these approaches carry inherent drawbacks, e.g., training the model in only one particular scenario may lead to overfitting, making it difficult for the model to be effectively transferred to new scenarios. Furthermore, they do not possess an effective mechanism for extracting generalized dynamical information from diverse scenarios.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/intro-two-sota2.pdf}
    \caption{Two state-of-the-art methods: (1) whether it's multi-agent and (2) whether it's multi-scenario.}
    \label{fig:intro-two-sota}
\end{figure}

% \revise{To conclude, there is so far no work guiding how to coordinate multi-agent across multi-scenario. \hl{It is challenging since simply putting a multi-agent model in a multi-scenario learning setting could experience devastatingly unstable training, which has already taken shape in the single-agent version, i.e., MetaLight.} To encourage a long-term dynamic, introducing temporal modules such as LSTM is expected to aggravate the unstable learning, given the history is already unstable. To this end, this work is dedicated to solving the following research question: \textbf{how to coordinate multi-agent across multi-scenario stably and with the ability to reserve long-term experience}.}

%To address the drawbacks of these two types of models, 
To tackle these challenges, we propose \textbf{DuaLight} with two modules: \textbf{scenario-shared co-train} and \textbf{scenario-specific experiential weights}. %This innovative framework enables concurrent learning from both the universal dynamics information across multiple scenarios and the environmental experiential information within a single scenario. 
%We formulate the coordination parameters as the intersection-wise and feature-wise weights, guiding how to aggregate neighboring intersections' information and different observation features, respectively.
(1) Co-Train module enables multi-scenario joint learning and to encourage stability, only a \textbf{subset} of the model's parameters is trained concurrently, yet the essential coordination parameters are learned within each scenario. (2) The experiential weight module  defines the coordination parameters as the intersection-wise and feature-wise weights, guiding how to aggregate neighboring intersections' information and different observation features, respectively. The two weights are trained after observing a whole episode, thus capturing the long-term dynamical experiences.

%This module can learn the environmental dynamic information about the neighbors and self-features within the scenario during training, which helps the model learn information that facilitates decision-making in a particular scenario. Specifically, this module can strengthen the experience information within a certain scenario by weighting the current neighbor observations and self-intersection observations.
%Additionally,  This module ensures the model's ability to extract the underlying dynamics information inherent across diverse scenarios.

The combination of these two modules encourages the model to learn and balance the shared dynamic information across multiple scenarios and the dynamic experiential information within a particular scenario, thus enabling the model to learn an effective representation to assist decision-making.

%%\jiang{最后列一下贡献点} check
In summary, this paper has three main contributions:
\begin{itemize}
    \item To the best of our knowledge, we are among the first to coordinate multi-agent across multi-scenario, with the consideration of both scenario-common and scenario-specific information by the co-train module and experiential weight module, respectively. 
    \item Specifically, we design the scenario-specific experiential weights that encourage modeling the influence of neighbors and input features, adaptive to different scenarios.
    \item We conduct experiments in both real-world and synthetic scenarios: DuaLight has the fastest and the most stable training and achieved the best results with 3-7\% improvements.
\end{itemize}
%First, the experiential weight module, which can learn the environmental dynamic information about neighbors and self-features within a particular scenario during training. Second, the Co-Train module, which enables the model to be trained across multiple scenarios, aims to learn the general dynamic information across different scenarios. Finally, we conduct experiments in both real-world and synthetic scenarios, where DuaLight achieved the best results or results close to the best across various metrics and scenarios.

